Smart Application for Fall Detection Using Wearable ECG & Accelerometer Sensors

Timely and reliable detection of falls is a large and rapidly growing field of research due to the medical and financial demand of caring for a constantly growing elderly population. Within the past 2 decades, the availability of high-quality hardware (high-quality sensors and AI microchips) and software (machine learning algorithms) technologies has served as a catalyst for this research by giving developers the capabilities to develop such systems. This study developed multiple application components in order to investigate the development challenges and choices for fall detection systems, and provide materials for future research. The smart application developed using this methodology was validated by the results from fall detection modelling experiments and model mobile deployment. The best performing model overall was the ResNet152 on a standardised, and shuffled dataset with a 2s window size which achieved 92.8% AUC, 87.28% sensitivity, and 98.33% specificity. Given these results it is evident that accelerometer and ECG sensors are beneficial for fall detection, and allow for the discrimination between falls and other activities. This study leaves a significant amount of room for improvement due to weaknesses identified in the resultant dataset. These improvements include using a labelling protocol for the critical phase of a fall, increasing the number of dataset samples, improving the test subject representation, and experimenting with frequency domain preprocessing.

==> conclusion/conclusion.tex <==
\chapter{Conclusion}

==> future-work/future-work.tex <==
\chapter{Recommendations for Future Work}

\section{Alternative Labelling Method}

\subsection{Critical Phase}
Use labelling that only marks the critical phase as a fall. This will allow us to use smaller window sizes implying less input features and ultimately lower complexity.

\section{Include Results of Deployed Model Inference Times}
This would be extremely useful to gauge and compare the complexity of varying models as a means to evaluate their reliability and suitability for fall detection in a commercial system.

\section{Alternative ECG Sensor Setup}

\subsection{Develop a small standalone wearable device}
The main limitation of this project along with the majority of biomedical systems is that of the usability. Although it is impossible to remove wearable devices completely (however this of course not the case of vision-based systems) we can try make them as minimal as possible, so they do not require regular charging and are not imposing on the appearance/comfort of the user.

This could be done by developing a self-contained system using analog nanotechnology. Analog chips are particularly relevant in this context due to their superior energy usage over digital chips, and the fact we are working with waveform data (accelerometer, and ECG sensors).

We could put ultimately put all the software on this chip and use techniques such as reservoir computing to optimise it for computing ML algorithms.

With regards to specific products this could be used in I thought a ring would be the most ideal due to its tiny footprint, and the fact it can easily be customised/designed to blend into (or even stand out from) a user's outfit.

\subsection{Use implant ECG sensors}
This could be useful for elderly with existing ECG implant sensors, as this would not require them to wear any additional external devices.

\subsection{Use optical ECG sensors on a smart watch}
This could be useful to prevent the requirement for the user to wear a chest strap constantly and have their phone on them. Rather it could all be integrated on a smart watch (ie. Apple Watch).

\section{Use other biometric readings}
\begin{itemize}
    \item Blood pressure - this would be extremely useful to detect whether users were about to faint by a significant drop/elevation in blood pressure.
    \item Blood glucose - this would be particularly useful for users with diabetes as it could detect whether users were about to faint due to a significant change of blood glucose. It could also include functionality to alert the user if their blood glucose drops below a certain threshold.
    \item Blood oxygen
    \item Respiration rate
    \item Skin temperature
    \item Extra user features: advanced biometrics (fat mass, bone mass, muscle mass, water), and medical conditions. 
\end{itemize}


\section{Abnormal Gait Detection}
Use this data to develop an abnormal gait detection model as a means to detect onset neurological conditions. For example detecting the freezing of gait experienced by a Parkinson's patient.

